CoDEx: Combining Domain Expertise for Spatial Generalization in Satellite Image Analysis

Global variations in terrain appearance raise a major challenge for satellite image analysis, leading to poor model performance when training on locations that differ from those encountered at test time. This remains true even with recent large global datasets. To address this challenge, we propose a novel domain-generalization framework for satellite images. Instead of trying to learn a single generalizable model, we train one expert model per training domain, while learning experts' similarity and encouraging similar experts to be consistent. A model selection module then identifies the most suitable experts for a given test sample and aggregates their predictions. Experiments on four datasets (DynamicEarthNet, MUDS, OSCD, and FMoW) demonstrate consistent gains over existing domain generalization and adaptation methods. Our code is publicly available at https://github.com/Abhishek19009/CoDEx.

==> figures/barplots.tex <==
%auto-ignore
\begin{tabular}{c@{}c@{}c@{}c@{}c}
\multicolumn{5}{c}{Test sets of datasets from GeoPlex}\\\greyrule
\begin{minipage}[t][4.35cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},
        width=1.2\linewidth,
        height=1\linewidth,
        title = {TreeSatAI-TS \\ {\vphantom{\vrule height 4mm width 0.1pt}} classif (weighted F1)},
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={AnySat, OmniSat, DOFA, PSE+LTAE},
        xtick={AnySat, OmniSat, DOFA,PSE+LTAE},
        xticklabels={\textbf{AnySat}, OmniSat, DOFA,PSE+LTAE},
        x tick label style={rotate=45, anchor=east, font=\footnotesize},
        y tick label style={font=\footnotesize},
        ytick={70,75},
        ymin=70.5,
        ymax=75,
        bar shift=-0pt,
    ] 
    % ANYSAT
    \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,75.1)};
    \addplot[fill=white] coordinates {(AnySat,72.6)}; 
    \addplot[fill=ANYCOLOR!20,draw=ANYCOLOR, very thick] coordinates {(AnySat,72.6)}; 

    % OMNISAT
    \addplot[fill=OMNICOLOR,draw=OMNICOLOR, very thick] coordinates {(OmniSat,74.2)};
    \addplot[fill=white] coordinates {(OmniSat,73.3)};
    \addplot[fill=OMNICOLOR!20,draw=OMNICOLOR, very thick] coordinates {(OmniSat,73.3)};

    % DOFA
    \addplot[fill=DOFACOLOR, draw=DOFACOLOR, very thick] coordinates {(DOFA,71.6)}; 

    % PSE+LTAE
    %\addplot[fill=DOFACOLOR] coordinates {(OmniSat,73.3)};
    \addplot[fill=TAECOLOR!20,draw=TAECOLOR, very thick] coordinates {(PSE+LTAE,71.2)};

    \end{axis}
\end{tikzpicture}
\end{minipage}
&
\begin{minipage}[t][4.35cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        title = {PASTIS-HD\\ {\vphantom{\vrule height 4mm width 0.1pt}} classif (macro F1)},
        width=1.2\linewidth,      
        height=1\linewidth,
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={AnySat, OmniSat, CROMA, DOFA},
        xtick={AnySat, OmniSat, CROMA, DOFA},
        xticklabels={\textbf{AnySat},\hphantom{\;}\hphantom{\;}\hphantom{\;} OmniSat, CROMA, DOFA},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=55.5,
        ymax=72,
        ytick={55,60,65,70},
        bar shift=-0pt,
    ] 

    %ANYSAT
    \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,72.8)};
    \addplot[fill=white] coordinates {(AnySat,65.5)};
    \addplot[fill=ANYCOLOR!20,draw=ANYCOLOR, very thick] coordinates {(AnySat,65.5)};

    % OMNISAT
    \addplot[fill=OMNICOLOR, draw=OMNICOLOR, very thick] coordinates {(OmniSat,69.9)};
    \addplot[fill=white] coordinates {(OmniSat,59.1)};
    \addplot[fill=OMNICOLOR!20,draw=OMNICOLOR, very thick] coordinates {(OmniSat,59.1)};

    % CROMA
    \addplot[fill=CROMACOLOR, draw=CROMACOLOR, very thick] coordinates {(CROMA,60.1)};

    % DOFA
    \addplot[fill=DOFACOLOR, draw=DOFACOLOR, very thick] coordinates {(DOFA,55.7)};

    \end{axis}
\end{tikzpicture}
\end{minipage}
&
\begin{minipage}[t][4.35cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        width=1.2\linewidth,  
      height=1\linewidth,
        title = {PLANTED \\ {\vphantom{\vrule height 4mm width 0.1pt}} classif (macro F1)},
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={ViViTS2, AnySat, ViViTMM},
        xtick={AnySat, ViViTS2, ViViTMM},
        xticklabels={\textbf{AnySat}, \textcolor{gray}{$^\star$ViViT-S2}, \textcolor{gray}{$^\star$ViViTS-MM}},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=55,
        ymax=65,
        bar shift=-0pt,
    ] 
    % ANYSAT
     \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,61.5)};
    \addplot[fill=white] coordinates {(AnySat,61.2)}; 
    \addplot[fill=ANYCOLOR!20, draw=ANYCOLOR, very thick] coordinates {(AnySat,61.2)};

    % ViViT
    
    \addplot[fill=TSVITCOLOR!20,draw=TSVITCOLOR, very thick] coordinates {(ViViTS2,62.2)};

    \addplot[fill=TSVITCOLOR!20,draw=TSVITCOLOR, very thick] coordinates {(ViViTMM,59.3)};

    % % OMNISAT
    % \addplot[fill=OMNICOLOR] coordinates {(OmniSat,74.2)};
    % \addplot[fill=white] coordinates {(OmniSat,73.3)};
    % \addplot[pattern color=OMNICOLOR, pattern=north east lines] coordinates {(OmniSat,73.3)};

    % % DOFA
    % \addplot[fill=DOFACOLOR] coordinates {(DOFA,71.6)}; 

    % % PSE+LTAE
    % %\addplot[fill=DOFACOLOR] coordinates {(OmniSat,73.3)};
    % \addplot[pattern color=TAECOLOR, pattern=north east lines] coordinates {(PSE+LTAE,71.2)};

    \end{axis}
\end{tikzpicture}
\end{minipage}
&
\begin{minipage}[t][4.35cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        width=1.2\linewidth,  
      height=1\linewidth,
        title = {PASTIS-HD\\ {\vphantom{\vrule height 4mm width 0.1pt}} semseg (mIoU)},
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={AnySat, UTAE-MM, TSViT,UTAE},
        xtick={AnySat, UTAE-MM, TSViT,UTAE},
        xticklabels={\textbf{AnySat}, UTAE-MM, TSViT,UTAE},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=63,
        ymax=66.55,
        bar shift=-0pt,
    ] 
    % ANYSAT
    \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,66.5)};
    \addplot[fill=white] coordinates {(AnySat,66.3)}; 
    \addplot[fill=ANYCOLOR!20,draw=ANYCOLOR, very thick] coordinates {(AnySat,66.5)}; 

    % UTAE
    \addplot[fill=TAECOLOR!20, draw=TAECOLOR, very thick] coordinates {(UTAE-MM,66.3)};

    % TSVITS
    \addplot[fill=TSVITCOLOR!20, draw=TSVITCOLOR, very thick] coordinates {(TSViT,65.4)};

     \addplot[fill=TAECOLOR!20, draw=TAECOLOR, very thick] coordinates {(UTAE,63.1)};
    \end{axis}
\end{tikzpicture}
\end{minipage}
&
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        title = {FLAIR\\ {\vphantom{\vrule height 4mm width 0.1pt}} semseg (mIoU)},
        width=1.2\linewidth,   
      height=1\linewidth,
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={UTT, AnySat,UNet, UTAE},
        xtick={AnySat,UTT, UNet, UTAE},
        xticklabels={\textbf{AnySat}, $^+$\textcolor{gray}{UT\&T},UNet, $^+$\textcolor{gray}{UTAE}},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=53,
        ymax=58,
        bar shift=-0pt,
    ] 
    % AnySat
    %\addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,55.6)};
    \addplot[fill=white] coordinates {(AnySat,55.6)};
    \addplot[fill=ANYCOLOR!20, draw=ANYCOLOR, very thick] coordinates {(AnySat,55.6)};

    % UT&T
    \addplot[fill=UTTCOLOR, draw=UTTCOLOR, very thick] coordinates {(UTT,56.9)};

    % UT\&T Mit-B2
    % \addplot[pattern color=UTTB2COLOR, pattern=north east lines] coordinates {(UTTMIT,62.6)};

    \addplot[draw=UNETCOLOR, fill=UNETCOLOR, very thick] coordinates {(UNet,54.7)};

    \addplot[fill=none, draw=none] coordinates {(UTAE,54.1)};
    \node[anchor=south, font=\footnotesize, text=black, inner sep=1pt] at (axis cs:UTAE,52.3) {36.1};
     
    \end{axis}
\end{tikzpicture}
\end{minipage}
\\[-5mm]
\multicolumn{5}{c}{External datasets}\\\greyrule
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
\begin{axis}[
    title style={align=center, font=\footnotesize},    
    legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
    title = {SICKLE\\ {\vphantom{\vrule height 4mm width 0.1pt}} semseg (IoU)},
    width=1.2\linewidth, 
  height=1\linewidth,
    ybar,
    bar width=15pt,
    enlargelimits=0.15,
    symbolic x coords={AnySat, THREEDUNET, THREEDUNETS2, UTAE},
    xtick={AnySat, THREEDUNET, THREEDUNETS2, UTAE},
    xticklabels={\textbf{AnySat}, 3DUNet-MM, 3DUNet-S2, UTAE},
    x tick label style={rotate=45, anchor=east, font=\footnotesize},         
    y tick label style={font=\footnotesize},
    ymin=71.8,
    ymax=90, % Tighter y-axis range
    bar shift=-0pt,
]

% ANYSAT
\addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,89.3)};
\addplot[fill=white] coordinates {(AnySat,82.0)};
\addplot[pattern color=ANYCOLOR, pattern=north east lines, very thick, draw=ANYCOLOR] coordinates {(AnySat,82.0)};
\draw[red, very thick] (axis cs:AnySat,82.0) ++ (-7.5pt,0) -- ++ (15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=red] {\bf 6.1K};

% 3D-MM
\addplot[fill=UNETCOLOR!20, draw=UNETCOLOR, very thick] coordinates {(THREEDUNET,82.1)};

% 3D-S2
\addplot[fill=UNETCOLOR!20, draw=UNETCOLOR, very thick] coordinates {(THREEDUNETS2,71.9)}; 

% Add a number instead of a bar for UTAE
\addplot[fill=none, draw=none] coordinates {(UTAE,71.9)};
\node[anchor=south, font=\footnotesize, text=black, inner sep=1pt] at (axis cs:UTAE,70) {51.4};
\end{axis}
\end{tikzpicture}
\vspace{5cm}
\end{minipage}
&
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        title = {BRADD-S1TS\\ {\vphantom{\vrule height 4mm width 0.1pt}} chgdet  (IoU)},
        width=1.2\linewidth, 
      height=1\linewidth,
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        %enlargelimits={abs, x=0.15, y=0.15},
        symbolic x coords={AnySat, UTAE, THREEDU, CONVLSTM},
        xtick={AnySat, UTAE, THREEDU, CONVLSTM},
        xticklabels={\textbf{AnySat}, UTAE, 3DUNet, ConvLSTM},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=62,
        ymax=81,
        bar shift=-0pt,
        ytick={60,70,80},
    ]

    %ANYSAT
    \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,80.9)};
    \addplot[fill=white] coordinates {(AnySat,78.9)};
    \addplot[pattern color=ANYCOLOR, pattern=north east lines, very thick, draw=ANYCOLOR] coordinates {(AnySat,78.9)};
    \draw[red, very thick] (axis cs:AnySat,78.9) ++ (-7.5pt,0) -- ++(15pt,0) ++ (+10pt,-2pt ) node[above, font=\scriptsize, color=red] { \bf 6.1K};   
    
    % UTAE
    \addplot[fill=TAECOLOR!20, draw=TAECOLOR, very thick] coordinates {(UTAE,70.7)}; 

     % UTAE-MM
    \addplot[fill=UNETCOLOR!20, draw=UNETCOLOR, very thick] coordinates {(THREEDU,68.1)}; 

    % UTAE-MM
    \addplot[fill=LSTMCOLOR!20, draw=LSTMCOLOR, very thick] coordinates {(CONVLSTM,63.1)}; 

    \end{axis}
\end{tikzpicture}
\vspace{5cm}
\end{minipage}
&
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        title = {TS2Crop\\ {\vphantom{\vrule height 4mm width 0.1pt}} classif (OA)},
        width=1.2\linewidth,
      height=1\linewidth,
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={AnySat, OSCNN, TAE, LSTM},
        xtick={AnySat, OSCNN, TAE, LSTM},
        xticklabels={\textbf{AnySat}, OS-CNN, TAE, LSTM},
                x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=72,
        ymax=95,
        bar shift=-0pt,
    ]
    %ANYSAT
    \addplot[fill=ANYCOLOR, draw=ANYCOLOR, very thick] coordinates {(AnySat,92.2)};
    \addplot[fill=white] coordinates {(AnySat,70.3)};
    \addplot[pattern color=ANYCOLOR, pattern=north east lines, very thick, draw=ANYCOLOR] coordinates {(AnySat,70.3)};
    \draw[red, very thick] (axis cs:AnySat,70.3) ++ (-7.5pt,0) -- ++(15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=red] {\bf 14K};  

    
    % OSCNN
    \addplot[fill=UNETCOLOR!20, draw=UNETCOLOR, very thick] coordinates {(OSCNN,81.2)}; 

     % v
    \addplot[fill=TAECOLOR!20, draw=TAECOLOR, very thick] coordinates {(TAE,80.9)}; 

     % LSTM
    \addplot[fill=LSTMCOLOR!20, draw=LSTMCOLOR, very thick] coordinates {(LSTM,78.2)}; 

    \end{axis}
\end{tikzpicture}
\vspace{5cm}
\end{minipage}
&
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\begin{tikzpicture}
    \begin{axis}[
        title style={align=center, font=\footnotesize},    legend style={at={(0.5,-0.15)},          anchor=north,legend columns=-1},,
        title = {Sen1Flood11\\ {\vphantom{\vrule height 4mm width 0.1pt}} semseg (mIoU)},
        width=1.2\linewidth,
      height=1\linewidth,
        ybar,
        bar width=15pt,
        enlargelimits=0.15,
        symbolic x coords={AnySat, CROMA, PRITHVI, SATLAS},
        xtick={AnySat, CROMA, PRITHVI,SATLAS},
        xticklabels={\textbf{AnySat}, CROMA, Prithvi, SatlasNet},
             x tick label style={rotate=45, anchor=east, font=\footnotesize},         y tick label style={font=\footnotesize},
        ymin=90,
        ymax=92,
        bar shift=-0pt,
    ]
    %ANYSAT
    \addplot[pattern color=ANYCOLOR, pattern=north east lines, very thick, draw=ANYCOLOR] coordinates {(AnySat,91.1)};
    \draw[red, very thick] (axis cs:AnySat,91.1) ++ (-7.5pt,0) -- ++(15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=red] { \bf 6.1K}; 

     % v
    \addplot[pattern color=CROMACOLOR, pattern=north east lines, draw=CROMACOLOR, very thick] coordinates {(CROMA,90.9)};
    \draw[black, very thick] (axis cs:CROMA,90.9) ++ (-7.5pt,0) -- ++(15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=black] {47M}; 

     % PRITHVI
    \addplot[pattern color=PRITHVICOLOR, pattern=north east lines, draw=PRITHVICOLOR, very thick] coordinates {(PRITHVI,90.4)};
    \draw[black, very thick] (axis cs:PRITHVI,90.4) ++ (-7.5pt,0) -- ++(15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=black] {39M};

       % SATLAS
    \addplot[pattern color=SATLASCOLOR, pattern=north east lines, draw=SATLASCOLOR, very thick] coordinates {(SATLAS,90.3)};
    \draw[black, very thick] (axis cs:SATLAS,90.3) ++ (-7.5pt,0) -- ++(15pt,0) ++ (-7.5pt,-2pt ) node[above=1.5mm, font=\scriptsize, color=black] {33M};

    \end{axis}
\end{tikzpicture}
\vspace{5cm}
\end{minipage}
&
\begin{minipage}[t][4.75cm][t]{.20\textwidth}\vspace{-3mm}
\raisebox{-2.5cm}{
\begin{tabular}{rl}
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)}]
     \fill [fill=ANYCOLOR!20, draw=ANYCOLOR, very thick] (0,0) rectangle (0.6,0.4);
\end{tikzpicture}
&\footnotesize
from scratch
\\[2mm]
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)}]
     \fill [draw=black,fill=ANYCOLOR, draw=ANYCOLOR, very thick] (0,0) rectangle (0.6,0.4);
\end{tikzpicture}
&\footnotesize
fine-tuned
\\[2mm]
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)}]
    \fill [pattern color=ANYCOLOR, pattern=north east lines, draw=black,draw=ANYCOLOR, very thick] (0,0) rectangle (0.6,0.4);
     \draw [red, very thick] (0,0.4) -- (0.6,0.4);
\end{tikzpicture}
&\footnotesize
linear probing
\\[2mm]
\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.north)}]
    \fill [pattern color=PRITHVICOLOR, pattern=north east lines, draw=black,draw=PRITHVICOLOR, very thick] (0,0) rectangle (0.6,0.4);
     \draw [black, very thick] (0,0.4) -- (0.6,0.4);
\end{tikzpicture}
&\footnotesize
UperNet probing
\\[2mm]
\begin{tikzpicture}[baseline={([yshift={-0.5*\ht\strutbox}]current bounding box.center)}]
     \draw [red, very thick] (0,0.0) -- (0.6,0.0);
     \node [draw=none] at (0.3,0.2) {\small \textcolor{red}{\bf 6.1K}};
\end{tikzpicture}
&\footnotesize  free parameters
\end{tabular}
}
%\vspace{5cm}
\end{minipage}
\\[-5mm]
\multicolumn{5}{c}{\centering
~\qquad $\star$ \textcolor{gray}{models trained on private external data}\qquad $+$ \textcolor{gray}{access to additional context}}
\end{tabular}

==> figures/pipeline.tex <==
%auto-ignore
\includegraphics[width=\linewidth, height=0.2\textheight]{example-image}

==> sections/999_experiments_bk.tex <==
%auto-ignore
We evaluate the performance of our proposed approach across four Earth Observation datasets (\cref{sec:data}, and compare it to a wide array of domain-generalization and adaptation methods (\cref{sec:results}). We also provide an ablation study in \cref{sec:ablation}.

%======================================
\subsection{Datasets and Evaluation}
\label{sec:data}
%======================================
\paragraph{DynamicEarthNet~\cite{toker2022dynamicearthnet}.} 
[A quick word about DynamicEarthNet: its nature, resolution, annotations, number of classes]
The data is split to represent 55 tiles (size 1024 x 1024) in the training set and 10 tiles in each validation/test set. We use features from each Encoder/Decoder layer of MultiHead MultiUTAE backbone as input to head selector. There are total of 6 classes for segmentation task and 4 spectral bands (RGB + NiR). Observations for 24 consecutive months are available for this dataset. 
\paragraph{MUDS~\cite{van2021multi}.} 
There are total of 40 tiles (size 1024 x 1024) in training set and a similar 10 tiles in validation/test set. There are only 2 classes (building and not building) with RGB spectral bands. For ground truth, we have binary segmentation maps as pixelwise annotations. Observations for 24 consecutive months are available for this dataset. 
\paragraph{OSCD~\cite{daudt2018urban}.} 
The dataset comprises 24 pairs of multispectral images taken from the Sentinel-2 satellites between years 2015 and 2018. Locations are selected for all over the world, in Brazil, USA, Europe, Middle-East and Asia. For each location, registered pairs of 13-band multispectral satellite images obtained by the Sentinel-2 satellites are provided. Images vary in spatial resolution between 10m, 20m and 60m. Pixel-level change ground truth is provided for all 14 training and 10 test image pairs. Annotations are available for buildings and roads. \\
\paragraph{FMoW-WILDS~\cite{christie2018functional, koh2021wilds}.}
The task is to predict building or land use category based on satellite images. We evaluate on subset of FMoW called FMoW-Asia, including 18 countries from Asia. Overall, FMoW-WILDS consists of over 1 million images from over 200 countries. The dataset is already segregated into train and test taking into account the spatial domain shift.

\paragraph{}

\begin{table*}[t]    
    \renewcommand{\arraystretch}{1.05}
    % \setlength{\tabcolsep}{3pt}
     \setlength{\fboxsep}{1.5pt}
    \caption{{\bf Quantitative Results.} We report the results of various domain generalization and adaptation we implemented and evaluated on 4 datasets. Cell color represent the \colorbox{green!50}{improved} or \colorbox{red!50}{decreased\vphantom{p}} performance with respect to the baseline. *Oracle results are reported only as a theoretical upper bound of how our DomainSelector can improve over the baseline, not for direct comparison.}
    \label{tab:main_results}
\input{tables/results}
\end{table*}

% \begin{table*}[htbp]
%     \centering
%     \setlength{\tabcolsep}{3pt} % Adjust column spacing
%     \renewcommand{\arraystretch}{1.2} % Adjust row spacing
%     \caption{Dataset Overview}
%     \arrayrulecolor[gray]{0.7} % Set the default table rules to grey
%     \begin{tabular}{@{}p{3cm}p{3cm}p{3cm}p{4cm}@{}}
%         \arrayrulecolor{black} % Top rules in black
%         \specialrule{1.2pt}{0pt}{0pt} % Thick top rule
%         \textbf{Name} & \textbf{Type} & \textbf{Dimensions (T x H x W x C)} & \textbf{Description} \\ 
%         \specialrule{1.2pt}{0pt}{0pt} % Thick second rule
%         \arrayrulecolor[gray]{0.7} % Set middle rules to grey
%         \multicolumn{4}{l}{\textbf{DynamicEarthNet}} \\
%         \quad planetfusion & float & (24, 1024, 1024, 4) & PlanetFusion RGB + Near Infrared \\ 
%         \midrule
%         \multicolumn{4}{l}{\textbf{MUDS}} \\
%         \quad planet & float & (24, 1024, 1024, 3) & Planet RGB \\ 
%         \midrule
%         \multicolumn{4}{l}{\textbf{Planted}} \\
%         \quad s1 & float & (8, 12, 12, 3) & Sentinel-1 backscatter \& look angle \\ 
%         \quad s2 & int & (8, 12, 12, 10) & Sentinel-2 reflectivity \\ 
%         \quad l7 & int & (20, 4, 4, 6) & Landsat-7 reflectivity \\ 
%         \quad modis & float & (60, 1, 1, 7) & MODIS reflectivity \& derivatives \\ 
%         \quad alos & float & (4, 4, 4, 3) & ALOS PALSAR backscatter \& look angle \\ 
%         \arrayrulecolor{black} % Reset bottom rule to black
%         \bottomrule
%     \end{tabular}
% \end{table*}



\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{images/qualitative_all.pdf}
    \caption{Qualitative results on DynamicEarthNet and Muds.}
    \label{fig:qualitative}
\end{figure*}

\textbf{Head Selection Performance} 
Table~\ref{tab:main_results} summarizes the results. The baseline is computed using the joint model (MultiUTAE). The Head Selector consistently outperforms the baseline across both metrics on the benchmark datasets. For DynamicEarthNet, \texttt{HS} improves mIoU and Accuracy by approximately 0.7 and 1.3, respectively. Similarly, for MUDS, \texttt{HS} achieves gains of around 0.6 for mIoU and 0.2 for Accuracy. The Oracle represents the theoretical upper bound on performance, achieved if the optimal head is selected for all SITS patches. \\

\textbf{Quantitative Results} 
Reported in Table \ref{tab:main_results}. \\

\textbf{Qualitative Results} Highlighted in Figure \ref{fig:qualitative}. \\

% % Define colors for legend
% \definecolor{impervious}{RGB}{128, 128, 128}
% \definecolor{agriculture}{RGB}{255, 204, 102}
% \definecolor{vegetation}{RGB}{0, 153, 0}
% \definecolor{wetlands}{RGB}{102, 204, 255}
% \definecolor{soil}{RGB}{153, 102, 51}
% \definecolor{water}{RGB}{0, 0, 255}
% \definecolor{notbuilding}{RGB}{240, 240, 240}
% \definecolor{building}{RGB}{255, 102, 102}

% \begin{figure*}
%     \centering
%     \renewcommand{\arraystretch}{1.3} % Adjust row spacing
%     \setlength{\tabcolsep}{2pt} % Adjust column spacing

%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{c c c c c c c c c c c}
%             & i & ii & iii & iv & v & vi & vii & viii & ix & x \\ 
            
%             \rotatebox{90}{Input} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png}\\
            
%             \rotatebox{90}{GT} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{example-image} &
%             \includegraphics[width=1.5cm]{example-image} & 
%             \includegraphics[width=1.5cm]{example-image}\\
            
%             \rotatebox{90}{Baseline} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png}\\
            
%             \rotatebox{90}{Ours} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} & 
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png} &
%             \includegraphics[width=1.5cm]{images/methodology/pred1.png} & \includegraphics[width=1.5cm]{images/methodology/pred1.png}\\
            
%         \end{tabular}
%     }
    
%     % Legend
%     \vspace{0.5cm}
%     \begin{tabular}{ccccccc}
%         \cellcolor{impervious} \hspace{0.5cm} & Impervious Surface &
%         \cellcolor{agriculture} \hspace{0.5cm} & Agriculture &
%         \cellcolor{vegetation} \hspace{0.5cm} & Vegetation \\
        
%         \cellcolor{wetlands} \hspace{0.5cm} & Wetlands &
%         \cellcolor{soil} \hspace{0.5cm} & Soil &
%         \cellcolor{water} \hspace{0.5cm} & Water \\
        
%         \cellcolor{notbuilding} \hspace{0.5cm} & Not Building &
%         \cellcolor{building} \hspace{0.5cm} & Building & \\
%     \end{tabular}

%     % Figure Caption
%     \caption{Qualitative results on DynamicEarthNet and Muds.}
% \end{figure*}


\textbf{Performance with different backbones} Summarized in Figure~\ref{fig:backbone}.

\input{tables/backbones.tex}


\FloatBarrier  % Requires \usepackage{placeins}



% \begin{tabular}{c@{}c@{}c@{}}
% \input{tables/backbones}
% \end{tabular}


\subsection{Ablation}
\textbf{Loss ablation for \texttt{HS}} We experimented with two loss objectives, mean square error (MSE) and mean error (L1) and evaluated head selection performance.

\textbf{Impact of \(p_{moh}\) vs \texttt{HS}} We experimented the impact of \(p_{moh}\) on the performance of domain generalization.

% \begin{table*}[t!]
% \centering
% \caption{Ablation Results}
% \label{tab:ablation_study}
% \begin{tabular}{l l cc cc}
% \toprule
% \multirow{2}{*}{\textbf{Settings}} & \multirow{2}{*}{\textbf{Variant}} & \multicolumn{2}{c}{\textbf{DynamicEarthNet}} & \multicolumn{2}{c}{\textbf{MUDS}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% & & \textbf{mIoU} & \textbf{OA} & \textbf{mIoU} & \textbf{OA} \\
% \midrule
% MSE + \( p_{moh} \) + MultiLevel Feats. & MSE Loss & 37.7 & 74.3 & 63.2 & 95.0 \\
% L1 + \texttt{HS} + MultiLevel Feats. & \texttt{HS} strategy & 36.5 & 73.6 & 62.9 & 94.4 \\
% L1 + \( p_{moh} \) + No Temp. Pooling & No Temp. Pool & 36.1 & 73.2 & 63.1 & 94.5 \\
% L1 + \( p_{moh} \) + Local Pooling (16×16) & Local Pool & 36.4 & 73.4 & 63.8 & 94.7 \\
% L1 + \( p_{moh} \) + MultiLevel Feats. + w/o Cons. Loss & w/o Cons. & 38.2 & 75.1 & 63.6 & 95.3 \\
% L1 + \( p_{moh} \) + MultiLevel Feats. + w Cons. Loss & w Cons. & \textbf{39.2} & \textbf{75.9} & \textbf{64.2} & \textbf{95.8} \\
% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[t!]
\centering
\caption{Head Selection Strategies and Settings (without consistency loss).}
\label{tab:ablation_study}
\begin{tabular}{l l l c cc cc}
\toprule
\textbf{Pooling} & \textbf{Loss} & \textbf{Features} & \textbf{Aggregation ($p_{moh}$)} & \multicolumn{2}{c}{\textbf{DynamicEarthNet}} & \multicolumn{2}{c}{\textbf{MUDS}} \\
\cmidrule(lr){5-6} \cmidrule(lr){7-8}
& & & & \textbf{mIoU} & \textbf{OA} & \textbf{mIoU} & \textbf{OA} \\
\midrule
Spatio-Temporal & L1 & MultiLevel  & \ding{56} & 36.5 & 73.6 & 62.9 & 94.4 \\
No Temporal & L1 & MultiLevel  & \ding{52} & 36.1 & 73.2 & 63.1 & 94.5 \\
Local (16×16) & L1 & MultiLevel & \ding{52} & 36.4 & 73.4 & 63.8 & 94.7 \\
Spatio-Temporal & MSE & MultiLevel  & \ding{52} & 37.7 & 74.3 & 63.2 & 95.0 \\
Spatio-Temporal & L1 & MultiLevel & \ding{52} & 38.2 & 75.1 & 63.6 & 95.3 \\

% Spatio-Temporal & L1 & MultiLevel & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.2} & \textbf{95.8} \\
\bottomrule
\end{tabular}
\end{table*}







==> sections/999_method_bk.tex <==
%auto-ignore
In this section we discuss some preliminaries followed by description of multihead network and head selector module.

\subsection{Preliminaries}
We address the problem of predicting the label \(y \in Y\) based on an input satellite image time series \(x \in X\). Given training data drawn from a distribution \(P_{\text{tr}}\), we train a model \(f\), parameterized by \(\theta\), using a loss function \(\ell\). Traditional empirical risk minimization (ERM) optimizes the following objective:  
\begin{equation}
\arg\min_{\theta \in \Theta} \mathbb{E}_{(x, y) \sim P_{\text{tr}}} \left[\ell(f_\theta(x), y)\right].
\end{equation}  
The trained model is evaluated on a test set sampled from a different distribution, \(P_{\text{ts}}\). When distribution shift occurs, the training and test distributions differ, i.e., \(P_{\text{tr}} \neq P_{\text{ts}}\).  

We consider a scenario where the overall data distribution is composed of a set of domains \(\mathcal{D} = \{1, \dots, D\}\), with each domain \(d \in \mathcal{D}\) associated with a domain-specific data distribution \(P_d\). Each domain provides a dataset \((X, Y, d) = \{(x_i, y_i, d)\}_{i=1}^{n_d}\). The training and test distributions are modeled as mixtures of the domain distributions:  
\[
P_{\text{tr}} = \sum_{d \in \mathcal{D}} \alpha_{\text{tr}, d} P_d \quad \text{and} \quad P_{\text{ts}} = \sum_{d \in \mathcal{D}} \alpha_{\text{ts}, d} P_d,
\]
where \(\alpha_{\text{tr}, d}\) and \(\alpha_{\text{ts}, d}\) represent the mixture probabilities for domains in the training and test sets, respectively.  

The sets of domains contributing to the training and test distributions are defined as:  

\begin{equation}
\begin{split}
\mathcal{D}_{\text{tr}} = \{d \in \mathcal{D} \mid \alpha_{\text{tr}, d} > 0\} \quad \text{and}\\ 
\quad \mathcal{D}_{\text{ts}} = \{d \in \mathcal{D} \mid \alpha_{\text{ts}, d} > 0\}.
\end{split}
\end{equation}

In this work, we focus on domain shifts where the test domains are disjoint from the training domains, i.e., \(\mathcal{D}_{\text{tr}} \cap \mathcal{D}_{\text{ts}} = \emptyset\).

\subsection{Multi-Head Network}

% \begin{figure*}
%     \centering
%     \includegraphics[width=15cm]{images/methodology_v3.pdf}
%     \caption{{\bf Pipeline.}}
%     \label{fig:enter-label}
% \end{figure*}

% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}{0.2\textwidth}
%         \centering
%         \begin{tikzpicture}[scale=0.9, transform shape]
%             \input{figures/methodA.tex} % Include first TikZ figure
%         \end{tikzpicture}
%         \label{fig:figure1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.2\textwidth}
%         \centering
%         \begin{tikzpicture}[scale=0.9, transform shape]
%             \input{figures/methodB.tex}
%         \end{tikzpicture}
%         \label{fig:figure2}
%     \end{subfigure}
%     \caption{Overall caption for both figures}
% \end{figure*}

\begin{figure*}
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row spacing if needed
    \begin{tabularx}{\textwidth}{X X} % Two equally distributed columns
        \begin{minipage}{0.48\textwidth} % Control figure width
            % \centering
            \begin{tikzpicture}[scale=0.9, transform shape]
                \input{figures/methodA.tex}
            \end{tikzpicture}
            \subcaption{Multi-Head Network}
        \end{minipage}
    &
        \begin{minipage}{0.48\textwidth} % Control figure width
            \centering
            \begin{tikzpicture}[scale=0.7, transform shape]
                \input{figures/methodB.tex}
            \end{tikzpicture}
            \subcaption{Head Selection Module}
        \end{minipage}
    \end{tabularx}
        \caption{Overview of methodology.  
    Here, \textcolor{black!40}{\small \faSnowflake} indicates frozen layers,  
    \textcircled{$\times$} represents vector multiplication.}

\end{figure*}



We introduce Multi-Head architecture to address the challenge of spatial domain shift. For the backbone of our architecture, we use MultiUTAE \cite{vincent2024satellite}, designed for satellite image time series segmentation and change detection. We can evaluate MultiUTAE on monodate dataset as well. The number of heads is determined by the sub-domains present in the train split. For the DynamicEarthNet dataset, we employ a 55-headed MultiUTAE, where each head is trained specifically on its corresponding sub-domain within the train split. To ensure comparable evaluation, the architecture of each head mirrors that of a single-head MultiUTAE.

The input to MM segmentation network is similar to MultiUTAE i.e., SITS \(x\) in \(\mathbb{R}^{T \times H' \times W' \times C}\) of T satellite images of spatial dimensions \(H' \times W'\) with C spectral bands. The encoder consists a series of successive down-sampling convolutions with multi-temporal attention map at the lowest resolution. We denote it by \(E\).
This is followed by a Decoder \(D\) with a series of strided-transposed convolutions to upsample the feature maps. We use a final convolution block to output per-pixel segmentation mask \(s\) \(\in\) \(\mathbb{R}^{H \times T \times H'\times W' 
\times K}\), where \(K\) is the number of semantic classes, \(H\) is the number of segmentation heads. 

In our framework, we keep the number of heads to be equivalent to the sub-domains in the training set. During training, we pass \(x\) of the sub-domain \(d_{h} \in {d_{1}, d_{2}, ..., d_{H}}\) through the corresponding head \(h\) and perform gradient descent at head \(h\). The encoder \(E\) and decoder \(D\) have shared parameters and specialization only happens in the final convolution block of each head. During inference, the ground-truth and sub-domain knowledge is usually not available, thus, we employ a head-selection strategy to select the best head using a light-weight head selector module.



\subsubsection{Training with Consistency Loss}

We experiment with a consistency regularizer loss in our multihead architecture inspired by \cite{yaoimproving}. The idea is to build a network where similar domains have similar predictive functions. This is done by utilizing coordinate information of domains. 
The weight \(a_{d}\) is determined using angle of the domain coordinates \(x_{d}\) = arctan\((x_{d, 2}/x_{d, 1})\). The angle difference between two domains \(x_{i}\) and \(x_{j}\) is computed as 
\(a^{g}_{ij}\) = arctan\((x_{j, 2}/x_{j, 1}\)) - arctan\((x_{i, 2}/x_{i, 1})\).

For the formulation of  relation-aware consistency loss, we can adopt two strategies: \\
\textbf{Strategy I}:
Computing \texttt{softmax} of the angles:
\[
a_d = \frac{\exp\left(\frac{a_d}{T}\right)}{\sum\limits_{d' = 1}^{D} \exp\left(\frac{a_{d'}}{T}\right)}
\]
The temperature is set as 1.0. Details can be found in ablation.
\\

\textbf{Strategy II}:
By directly utilizing them as weights.
Consistency regularization can be formulated as:

\[
L_{\text{rel}} = \mathbb{E}_{d \in D, (x,y) \sim P_d}
\left[ \ell
\left(
\frac{\sum\limits_{\substack{j=1, j \neq d}}^{D} a_{dj} f(j)(x)}
{\sum\limits_{\substack{k=1, k \neq d}}^{D} a_{dk}}
, y
\right) \right]
\]

\subsection{Head Selection Module}

For head selection, a lightweight module is implemented that processes the feature output from multi-level feature layers (encoder, decoder, input) of Multi-UTAE. Features are passed by a simple convolutional block consisting of three convolution layers, which maps the spatio-temporal features to the appropriate head. Finally, global spatial-temporal pooling is performed. Performance of MM is evaluated against small (\(\sim\) 463K parameters) version of MultiUTAE.

Following \cite{vincent2024satellite}, each 1024 x 1024 tile of a subdomain is divided into 128 x 128 patches. This results in 64 time series per subdomain used to train the corresponding head of MM. An oracle is used to compute targets for the head selector. The oracle operates under the assumption that pixel-wise annotations are available for the train split, which is typically the case in supervised learning tasks. Specifically, the oracle uses a pretrained MM to compare the segmentation predictions of each head with the ground truth pixel segmentation mask. 

To train the head selector, we utilize an oracle to derive the performance of each head \(h\), represented as \(P \in \mathbb{R}^H\), where \(H\) is the total number of heads in the multi-head SITS segmentation network. The head selection network generates logits for a given SITS input \(x\), which are optimized using the Mean Error (ME) loss, defined as follows (see Equation \ref{meloss}): 

\begin{equation}
\label{meloss}
L_{ME} = |\texttt{HS(x)} - P|
\end{equation}

We incorporate a mixture of posterior probabilities from each head of the multi-head segmentation model. 
To transform \(\texttt{HS(x)}\) into a probability distribution, we apply the softmax function with temperature \(T=1\). This ensures that the outputs of \(\texttt{HS(x)}\) are normalized to represent probabilities, where each value falls between 0 and 1, and the sum of all probabilities equals 1. The softmax transformation is defined as follows:

\begin{equation}
\texttt{HS}_i(x) = \frac{\exp({\texttt{HS}_i(x)}/T)}{\sum_{j=1}^H \exp(\texttt{HS}_j(x)/T)}
\end{equation}


Here, \(\texttt{HS}_i(x)\) represents the \(i\)-th logit corresponding to head \(h_i\), and \(H\) is the total number of heads in the multi-head segmentation network. This transformation ensures that the logits \(\texttt{HS}(x)\) are converted into a valid probability distribution, which reflects the relative confidence in the performance of each head.

The metric \(\texttt{HS}(x)\) is used to quantify the confidence in each posterior probability for a specific input SITS \(x\) to give \(p_{moh}\) in \ref{pmoh}. Firstly, \(\texttt{HS}(x)\) is transformed to represent a probability distribution using softmax with temperature \(T=1\).


\begin{equation}
\label{pmoh}
p_{moh} = \sum_{h=1}^{H} \texttt{HS}_{h}(x) \cdot p_{h}
\end{equation}

where \(p_{h}\) is the posterior probability of softmax for the head \(h\).

The mixture of probabilities are optimized using the standard focal loss in equation \ref{focalloss_moh} based on the ground truth SITS mask.

\begin{equation}
\label{focalloss_moh}
\begin{split}
L_{FL}(p_{moh}, g, \gamma) = 
& -\sum_{t=1}^{T} \sum_{n=1}^{N} (1 - g^{nt} \cdot p_{moh}^{nt})^\gamma \\
& \cdot \log(g^{nt} \cdot p_{moh}^{nt})
\end{split}
\end{equation}


where \(g^{nt}\) represents the one-hot encoding vector representing the target class of the \(n^{th}\) pixel at the \(t\) time step, \(p_{moh}^{nt}\) represents the mixture of probability of the \(n^{th}\) pixel at the \(t\) time step.

Final objective of the head selector \(L_{\texttt{HS}}\) is the weighted combination of \ref{pmoh} and \ref{focalloss_moh}.

\begin{equation}
    \label{loss_comb}
L_{\texttt{HS}} = L_{ME} + \lambda^{'} \cdot L_{moh}
\end{equation}




==> sections/misc.tex <==
%auto-ignore

% No Temporal & L1 & \ding{56}  & \ding{52} & 36.1 & 73.2 & 63.1 & 94.5 \\

% Local (16×16) & L1 & \ding{56} & \ding{52} & 36.4 & 73.4 & 63.8 & 94.7 \\




% Spatio-Temporal & L1 & MultiLevel & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.2} & \textbf{95.8} \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Ablation study.}
% \label{tab:hswocl}
% \begin{tabular}{l l c c cc cc}
% \toprule
% \textbf{Pooling} & \textbf{\(\cLacc\)} & \textbf{Cons. Loss} & \textbf{$\cLmix$} & \multicolumn{2}{c}{\textbf{DynamicEarthNet}} & \multicolumn{2}{c}{\textbf{MUDS}} \\
% \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% & & & & \textbf{mIoU} & \textbf{OA} & \textbf{mIoU} & \textbf{OA} \\
% \midrule
% Spatio-Temporal & L1 & \ding{52} & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.3} & \textbf{95.7} \\
% Spatio-Temporal & L2 & \ding{52}  & \ding{52} & 38.7 & 75.1 & 64.0 & 94.8 \\
% Local (16×16) & L1 & \ding{52} & \ding{52} & 37.2 & 74.3 & 63.9 & 94.7 \\
% No Temporal & L1 & \ding{52}  & \ding{52} & 37.3 & 74.2 & 63.7 & 94.6 \\
% Spatio-Temporal & L1 & \ding{56} & \ding{52} & 38.2 & 75.1 & 63.6 & 95.3 \\
% Spatio-Temporal & L1 & \ding{52}  & \ding{56} & 38.4 & 75.0 & 64.1 & 94.8 \\
% Spatio-Temporal & L1 & \ding{56}  & \ding{56} & 36.5 & 73.6 & 62.9 & 94.4 \\

% No Temporal & L1 & \ding{56}  & \ding{52} & 36.1 & 73.2 & 63.1 & 94.5 \\

% Local (16×16) & L1 & \ding{56} & \ding{52} & 36.4 & 73.4 & 63.8 & 94.7 \\




% Spatio-Temporal & L1 & MultiLevel & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.2} & \textbf{95.8} \\




% \begin{table*}[t!]
% \centering
% \caption{Head Selection Strategies and Settings (with consistency loss).}
% \label{tab:hscl}
% \begin{tabular}{l l c c cc cc}
% \toprule
% \textbf{Pooling} & \textbf{Loss} & \textbf{Cons. Loss} & \textbf{Aggregation ($p_{moh}$)} & \multicolumn{2}{c}{\textbf{DynamicEarthNet}} & \multicolumn{2}{c}{\textbf{MUDS}} \\
% \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% & & & & \textbf{mIoU} & \textbf{OA} & \textbf{mIoU} & \textbf{OA} \\
% \midrule
% Spatio-Temporal & L1 & \ding{52}  & \ding{56} & 38.4 & 75.0 & 64.1 & 94.8 \\
% No Temporal & L1 & \ding{52}  & \ding{52} & 37.3 & 74.2 & 63.7 & 94.6 \\
% Local (16×16) & L1 & \ding{52} & \ding{52} & 37.2 & 74.3 & 63.9 & 94.7 \\
% Spatio-Temporal & MSE & \ding{52}  & \ding{52} & 38.7 & 75.1 & 64.0 & 94.8 \\
% Spatio-Temporal & L1 & \ding{52} & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.3} & \textbf{95.7} \\

% % Spatio-Temporal & L1 & MultiLevel & \ding{52} & \textbf{39.2} & \textbf{75.9} & \textbf{64.2} & \textbf{95.8} \\
% \bottomrule
% \end{tabular}
% \end{table*}




==> suppmat.tex <==
%auto-ignore
\renewcommand\thefigure{A-\arabic{figure}}
\renewcommand\thesection{A-\arabic{section}}
\renewcommand\thetable{A-\arabic{table}}
\renewcommand\theequation{A-\arabic{equation}}
\renewcommand\thealgorithm{A-\arabic{algorithm}}

==> tables/ablation_bk.tex <==
%auto-ignore
\begin{table*}[t!]
\centering
\begin{tabular}{l c c c c c cc cc}
\toprule
&\multirow{2}{*}{\textbf{$\cLcon$}} & \textbf{Spatial} & \textbf{Temporal} & \multirow{2}{*}{\textbf{$\cLmix$}} & \multirow{2}{*}{\textbf{\(\cLacc\)}} & \multicolumn{2}{c}{\textbf{DynamicEarthNet}} & \multicolumn{2}{c}{\textbf{MUDS}} \\
\cmidrule(lr){7-8} \cmidrule(lr){9-10}
&& \textbf{pooling} & \textbf{pooling} & & & \textbf{mIoU} & \textbf{OA} & \textbf{mIoU} & \textbf{OA} \\
\midrule
Best configuration & \ding{52} & \ding{52} & \ding{52} & \ding{52} & L1 & \textbf{39.2} & \textbf{75.9} & \textbf{64.3} & \textbf{95.7} \\
$\cLacc$ with L2 & \ding{52} & \ding{52} & \ding{52} & \ding{52}  & L2 & 38.7 & 75.1 & 64.0 & 94.8 \\
No Temporal pooling & \ding{52} & \ding{52} & & \ding{52}  & L1 & 37.3 & 74.2 & 63.7 & 94.6 \\
No $\cLcon$ & & \ding{52} & \ding{52} & \ding{52} & L1 & 38.2 & 75.1 & 63.6 & 95.3 \\
No $\cLmix$ & \ding{52} & \ding{52} & \ding{52} &   & L1 & 38.4 & 75.0 & 64.1 & 94.8 \\
No $\cLmix$ and $\cLcon$  & &\ding{52} & \ding{52} &   & L1 & 36.5 & 73.6 & 62.9 & 94.4 \\
\bottomrule
\end{tabular}

\caption{Ablation study.}
\label{tab:ablation}
\end{table*}


==> tables/ours_oracle_baseline.tex <==
%auto-ignore
\subsection{Baseline and Comparisons}
\begin{table*}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.3} % Adjust row spacing
    \setlength{\tabcolsep}{3pt} % Adjust column spacing
    \caption{Head Selector Performance. Bold is best. Underline is second best.}
    \label{hsperf}
    \arrayrulecolor[gray]{0.7} % Set the internal rules to grey
    \begin{tabular}{@{}p{3cm}p{2cm}p{2cm}p{2cm}p{2cm}@{}}
        \arrayrulecolor{black} % Top rules in black
        \specialrule{1.2pt}{0pt}{0pt} % Thick top rule
        \textbf{Dataset} & \textbf{Metric} & \textbf{\texttt{Ours}} & \textbf{Baseline} & \textbf{Oracle} \\
        \specialrule{1.2pt}{0pt}{0pt} % Thick second rule
        \arrayrulecolor[gray]{0.7} % Internal rules in grey
        \multirow{2}{*}{DynamicEarthNet} 
        & mIoU & \underline{38.2} & 37.5 & \textbf{48.7} \\ 
        & Acc & \underline{75.1} & 73.8 & \textbf{82.4} \\ 
        \midrule
        \multirow{2}{*}{MUDS} 
        & mIoU & \underline{64.2} & 63.5 & \textbf{66.2} \\ 
        & Acc & \underline{95.3} & 95.1 & \textbf{96.1} \\ 
        \midrule
        OSCD 
        & mIoU & \underline{35.6} & 32.7 & \textbf{41.5} \\ 
        & SC & \underline{23.7} & 21.5 & \textbf{32.5} \\
        \midrule
        FMoW-WILDS
        & Acc & \underline{77.2} & 73.4 & \textbf{82.4} \\
        \arrayrulecolor{black} % Bottom rules back to black
        \bottomrule
    \end{tabular}
\end{table*}
